Just MLPs: Efficient Visual State Reconstruction for Multimodal Language Models

Long visual token sequences often account for a substantial fraction of the computational overhead in multimodal large language models~(MLLMs). Existing approaches reduce this cost by pruning redundant visual tokens, but permanently discard visual evidence that may become useful in subsequent layers. We instead ask whether all visual tokens can be preserved while reducing the cost of repeatedly evolving the representations through the Transformer. To answer this question, we perform low-rank interventions on visual-to-text information flow. We find that, after visual-to-text attention is blocked, restoring only a few directions recovers most of the lost accuracy, suggesting the relevant visual influence is concentrated in a low-dimensional subspace. We further observe strong predictability in layer-specific visual states: lightweight MLPs approximate them with high cosine similarity and low reconstruction error. Motivated by these findings, we propose $\delta$-Vision, which replaces repeated Transformer evolution of visual tokens with lightweight low-rank adapters that construct layer-wise visual memories while preserving all visual tokens for text retrieval. Across image and video benchmarks, $\delta$-Vision achieves higher accuracy than visual token pruning baselines at comparable or lower computation, while delivering competitive inference efficiency without discarding visual tokens.

==> tables/attention_output_low_rank_acc.tex <==
\begin{table*}[htbp]
    \centering
    \caption{
    Performance comparison under different low-rank approximations on Qwen3-VL-4B and LLaVA-1.5-7B.
    }
    \label{tab:attention_output_low_rank_acc}
    \resizebox{\textwidth}{!}{%
    \renewcommand{\arraystretch}{1.15}
    \begin{tabular}{llccccccccc}
        \toprule
        \textbf{Model}
        & \textbf{Benchmark}
        & \textbf{Vanilla}
        & $\mathbf{r=0}$
        & $\mathbf{r=16}$
        & $\mathbf{r=32}$
        & $\mathbf{r=64}$
        & $\mathbf{r=128}$
        & $\mathbf{r=256}$
        & $\mathbf{r=512}$
        & $\mathbf{r=1024}$ \\
        \midrule

        % ==================== Qwen3-VL-4B ====================
        \rowcolor{gray!15}
        \multicolumn{11}{c}{\textbf{Qwen3-VL-4B}} \\

        Qwen3-VL-4B
        & SQA
        & 93.3
        & 72.0
        & 84.8
        & 89.0
        & 90.9
        & 92.2
        & 92.1
        & 92.8
        & 93.9 \\

        Qwen3-VL-4B
        & RWQA
        & 71.2
        & 46.3
        & 62.6
        & 65.9
        & 67.2
        & 69.9
        & 70.5
        & 71.5
        & 71.4 \\

        Qwen3-VL-4B
        & MMStar
        & 64.9
        & 25.2
        & 51.2
        & 56.8
        & 60.1
        & 61.0
        & 61.8
        & 63.8
        & 64.5 \\

        \midrule

        % ==================== LLaVA-1.5-7B ====================
        \rowcolor{gray!15}
        \multicolumn{11}{c}{\textbf{LLaVA-1.5-7B}} \\

        LLaVA-1.5-7B
        & SQA
        & 65.6
        & 62.9
        & 64.9
        & 66.1
        & 65.8
        & 65.5
        & 66.0
        & 65.8
        & 65.6 \\

        LLaVA-1.5-7B
        & RWQA
        & 54.9
        & 42.0
        & 51.9
        & 53.7
        & 54.1
        & 55.7
        & 55.2
        & 55.8
        & 56.1 \\

        LLaVA-1.5-7B
        & MMStar
        & 37.0
        & 24.9
        & 33.7
        & 34.9
        & 34.5
        & 35.3
        & 36.3
        & 36.4
        & 36.2 \\

        \bottomrule
    \end{tabular}%
    }
\end{table*}

==> tables/hidden_compress.tex <==
\begin{table*}[htbp]
    \centering
    \caption{
    Accuracy under different low-rank approximations of the visual effect.
    The full hidden dimensions are 2560 for Qwen3-VL-4B and 4096 for
    LLaVA-1.5-7B. \textit{Vanilla} denotes the accuracy of the original model.
    }
    \label{tab:rank_recovery}
    \resizebox{0.9\textwidth}{!}{%
    \renewcommand{\arraystretch}{1.15}
    \begin{tabular}{lcccccccc}
        \toprule
        \textbf{Dataset}
        & \textbf{Vanilla}
        & $\mathbf{r=0}$
        & $\mathbf{r=32}$
        & $\mathbf{r=64}$
        & $\mathbf{r=128}$
        & $\mathbf{r=256}$
        & $\mathbf{r=512}$
        & $\mathbf{r=1024}$ \\
        \midrule

        % ==================== Qwen3-VL-4B ====================
        \rowcolor{gray!15}
        \multicolumn{9}{c}{
            \textbf{Qwen3-VL-4B} \quad
            \textit{(Full hidden dimension: 2560)}
        } \\

        SQA
        & 91.70
        & 71.80
        & 73.50
        & 76.80
        & 84.20
        & 86.90
        & 89.40
        & 91.40 \\

        RealWorldQA
        & 70.72
        & 35.56
        & 42.09
        & 56.08
        & 63.14
        & 65.88
        & 67.97
        & 69.41 \\

        MMStar
        & 64.10
        & 23.80
        & 35.50
        & 46.30
        & 53.10
        & 58.70
        & 61.50
        & 64.50 \\

        \midrule

        % ==================== LLaVA-1.5-7B ====================
        \rowcolor{gray!15}
        \multicolumn{9}{c}{
            \textbf{LLaVA-1.5-7B} \quad
            \textit{(Full hidden dimension: 4096)}
        } \\

        SQA
        & 65.60
        & 59.70
        & 63.90
        & 65.80
        & 66.10
        & 66.20
        & 66.20
        & 66.30 \\

        RealWorldQA
        & 55.03
        & 40.26
        & 44.05
        & 49.15
        & 52.55
        & 54.64
        & 53.86
        & 54.77 \\

        MMStar
        & 37.00
        & 23.10
        & 29.90
        & 32.90
        & 35.80
        & 34.80
        & 35.70
        & 37.20 \\

        \bottomrule
    \end{tabular}%
    }
\end{table*}

==> tables/per_layer_mlp_predict.tex <==
\begin{table*}[htbp]
    \centering
    \caption{
    Layer-wise reconstruction quality of independently trained residual MLPs
    after 2,000 training steps.
    Layer indices start from 0.
    We report cosine similarity and mean squared error (MSE) on
    RealWorldQA, MMStar, and SQA.
    }
    \label{tab:layerwise_residual_mlp}
    \resizebox{0.86\textwidth}{!}{%
    \renewcommand{\arraystretch}{1.10}
    \begin{tabular}{c|cc|cc|cc}
        \toprule
        \multirow{2}{*}{\textbf{Layer}}
        & \multicolumn{2}{c|}{\textbf{RealWorldQA}}
        & \multicolumn{2}{c|}{\textbf{MMStar}}
        & \multicolumn{2}{c}{\textbf{SQA}} \\
        \cmidrule(lr){2-3}
        \cmidrule(lr){4-5}
        \cmidrule(lr){6-7}
        & \textbf{Cosine} & \textbf{MSE}
        & \textbf{Cosine} & \textbf{MSE}
        & \textbf{Cosine} & \textbf{MSE} \\
        \midrule

         0 & 1.0000 & 0.000000 & 1.0000 & 0.000000 & 1.0000 & 0.000000 \\
         1 & 0.9785 & 0.000094 & 0.9805 & 0.000086 & 0.9759 & 0.000107 \\
         2 & 0.9671 & 0.000285 & 0.9695 & 0.000274 & 0.9623 & 0.000341 \\
         3 & 0.9649 & 0.000493 & 0.9680 & 0.000481 & 0.9604 & 0.000607 \\
         4 & 0.9534 & 0.000982 & 0.9544 & 0.001041 & 0.9431 & 0.001321 \\
         5 & 0.9454 & 0.001170 & 0.9469 & 0.001270 & 0.9341 & 0.001625 \\
         6 & 0.9323 & 0.002523 & 0.9346 & 0.002798 & 0.9196 & 0.003611 \\
         7 & 0.9325 & 0.005507 & 0.9336 & 0.006068 & 0.9174 & 0.007898 \\
         8 & 0.9040 & 0.010207 & 0.9063 & 0.010943 & 0.8834 & 0.014229 \\
         9 & 0.8876 & 0.013396 & 0.8890 & 0.014774 & 0.8618 & 0.019340 \\
        10 & 0.8618 & 0.027698 & 0.8577 & 0.030642 & 0.8269 & 0.038764 \\
        11 & 0.8463 & 0.015788 & 0.8431 & 0.017260 & 0.8125 & 0.021713 \\
        12 & 0.8550 & 0.020102 & 0.8477 & 0.022037 & 0.8151 & 0.027825 \\
        13 & 0.8286 & 0.017769 & 0.8277 & 0.018828 & 0.7920 & 0.023735 \\
        14 & 0.8493 & 0.036829 & 0.8518 & 0.037594 & 0.8191 & 0.046762 \\
        15 & 0.8177 & 0.041455 & 0.8315 & 0.040756 & 0.7993 & 0.049554 \\
        16 & 0.7767 & 0.084378 & 0.7931 & 0.081547 & 0.7597 & 0.096644 \\
        17 & 0.7689 & 0.071098 & 0.7898 & 0.068677 & 0.7572 & 0.082283 \\
        18 & 0.7928 & 0.088414 & 0.8159 & 0.085635 & 0.7877 & 0.100764 \\
        19 & 0.8116 & 0.146896 & 0.8302 & 0.139159 & 0.8046 & 0.163698 \\
        20 & 0.8157 & 0.123455 & 0.8365 & 0.113062 & 0.8116 & 0.135634 \\
        21 & 0.8376 & 0.168068 & 0.8573 & 0.151308 & 0.8344 & 0.180399 \\
        22 & 0.8298 & 0.304275 & 0.8471 & 0.275573 & 0.8231 & 0.329826 \\
        23 & 0.8225 & 0.284698 & 0.8421 & 0.255275 & 0.8170 & 0.306142 \\
        24 & 0.8220 & 0.435841 & 0.8391 & 0.396900 & 0.8150 & 0.469354 \\
        25 & 0.8294 & 0.367051 & 0.8427 & 0.337816 & 0.8198 & 0.395020 \\
        26 & 0.8029 & 0.580795 & 0.8159 & 0.539481 & 0.7900 & 0.626982 \\
        27 & 0.8034 & 0.761241 & 0.8165 & 0.706911 & 0.7925 & 0.809480 \\
        28 & 0.8192 & 0.851573 & 0.8362 & 0.767666 & 0.8133 & 0.877876 \\
        29 & 0.7721 & 1.683211 & 0.7885 & 1.525666 & 0.7626 & 1.739717 \\
        30 & 0.7599 & 2.381083 & 0.7748 & 2.229408 & 0.7487 & 2.490592 \\
        31 & 0.7526 & 3.161811 & 0.7655 & 2.899676 & 0.7436 & 3.270941 \\
        32 & 0.7488 & 4.531008 & 0.7611 & 4.234886 & 0.7407 & 4.764305 \\
        33 & 0.7013 & 8.760635 & 0.7170 & 8.157923 & 0.6951 & 9.236602 \\
        34 & 0.7163 & 9.488822 & 0.7276 & 8.994737 & 0.7080 & 9.870068 \\
        35 & 0.6887 & 6.768492 & 0.6925 & 6.652475 & 0.6716 & 7.081798 \\

        \bottomrule
    \end{tabular}%
    }
\end{table*}

==> tables/rank_ablation.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{6pt}
\begin{tabular}{lcccccccccc}
\toprule
\textbf{Method} 
& \textbf{MMStar} 
& \textbf{RWQA} 
& \textbf{GQA} 
& \textbf{MMB} 
& \textbf{MMB-CN} 
& \textbf{MME} 
& \textbf{POPE} 
& \textbf{SQA} 
& \textbf{VQA-v2} 
& \textbf{Avg.} \\
\midrule

Qwen3-VL-4B
& 64.9 & 71.2 & 61.6 & 87.5 & 87.7
& 84.7 & 89.3 & 93.3 & 80.9 & 80.1 \\

Rank32
& 53.10 & 63.27 & 55.50 & 83.10 & 81.80
& 79.00 & 86.90 & 81.30 & 77.52 & 73.50 \\

Rank64
& 53.50 & 63.79 & 55.60 & 83.40 & 82.20
& 79.80 & 87.10 & 81.70 & 77.72 & 73.87 \\

$\delta$-Vision (Emb. Adapter)
& 54.4 & 62.9 & 56.7 & 84.5 & 82.8
& 80.1 & 87.6 & 82.3 & 78.0 & 74.4 \\

Rank256
& 54.60 & 64.71 & 55.30 & 83.80 & 82.60
& 79.70 & 86.90 & 80.90 & 77.54 & 74.01 \\

Rank512
& 55.40 & 63.27 & 57.30 & 84.00 & 82.90
& 79.60 & 87.30 & 82.10 & 77.37 & 74.36 \\

Rank1024
& 55.60 & 64.18 & 57.20 & 84.30 & 83.60
& 78.70 & 87.40 & 81.90 & 77.74 & 74.51 \\

\bottomrule
\end{tabular}
\caption{Performance comparison across different adapter ranks.}
\label{tab:rank_ablation
}
\end{table}

==> tables/visual_attention_ablation.tex <==
\begin{table}[htbp]
    \centering
    \caption{
    Ablation of visual information flow and residual recovery.
    \textit{Self-only} restricts visual tokens to self-interaction, while
    \textit{No Visual Attention} removes direct visual attention.
    \textit{Full Residual (2K)} denotes the residual module after 2,000
    training steps. All results are accuracy (\%).
    }
    \label{tab:visual_attention_ablation}
    \resizebox{0.82\textwidth}{!}{%
    \renewcommand{\arraystretch}{1.15}
    \begin{tabular}{lccc}
        \toprule
        \textbf{Method}
        & \textbf{RealWorldQA}
        & \textbf{MMStar}
        & \textbf{SQA} \\
        \midrule

        % ==================== Qwen ====================
        \rowcolor{gray!15}
        \multicolumn{4}{c}{\textbf{Qwen3-VL-4B}} \\

        Vanilla
        & 70.72
        & 64.10
        & 91.70 \\

        Self-only
        & 32.42
        & 49.30
        & 78.40 \\

        No Visual Attention
        & 47.19
        & 46.00
        & 76.50 \\

        Full Residual (2K)
        & 61.57
        & 52.80
        & 78.70 \\

        \addlinespace[2pt]

        $\Delta$ vs.\ No Visual Attention
        & +14.38
        & +6.80
        & +2.20 \\

        $\Delta$ vs.\ Vanilla
        & -9.15
        & -11.30
        & -13.00 \\

        \midrule

        % ==================== LLaVA ====================
        \rowcolor{gray!15}
        \multicolumn{4}{c}{\textbf{LLaVA-1.5-7B}} \\

        Vanilla
        & 54.64
        & 37.00
        & 65.60 \\

        Self-only
        & 49.41
        & 37.60
        & 64.20 \\

        No Visual Attention
        & 48.24
        & 35.40
        & 64.90 \\

        \bottomrule
    \end{tabular}%
    }
\end{table}
